Constrained Langevin Algorithms with L-mixing External Random Variables

Langevin algorithms are gradient descent methods augmented with additive noise, and are widely used in Markov Chain Monte Carlo (MCMC) sampling, optimization, and machine learning. In recent years, the non-asymptotic analysis of Langevin algorithms for non-convex learning has been extensively explored. For constrained problems with non-convex losses over a compact convex domain with IID data variables, the projected Langevin algorithm achieves a deviation of $O(T^{-1/4} (\log T)^{1/2})$ from its target distribution [27] in $1$-Wasserstein distance. In this paper, we obtain a deviation of $O(T^{-1/2} \log T)$ in $1$-Wasserstein distance for non-convex losses with $L$-mixing data variables and polyhedral constraints (which are not necessarily bounded). This improves on the previous bound for constrained problems and matches the best-known bound for unconstrained problems.

==> boundConstants.tex <==
\section{Bound the constants}

In this section, we bound the main constants 
$c_{\ref{contraction_const1}}, c_{\ref{contraction_const2}}, c_{\ref{error_polyhedron1}}, c_{\ref{error_polyhedron2}}  $
 shown in Theorem 1 so that we can have the simplified version of Theorem 1, which is loose but is easier for the application of optimization.



\begin{proposition}
\end{proposition}

\begin{proof}

Trace back to the contraction proof in


Here we show the constants explicitly so that we can see the dimension and parameter dependencies directly.

Combining the bound shown in line 674 and line 676 gives
\begin{align*}
\xi &\ge (R_1 - R_0) \Phi(R_1) \varphi(R_0)^{-1}/2\\
&\ge (R_1 - R_0) R_1e^{-h(R_0)} \varphi(R_0)^{-1}/2\\
& = (R_1 - R_0) R_1/2
\end{align*}

Here we choose $R_0 = R$.
and $R_1 = \frac{R}{2} +\frac{1}{2} \sqrt{R^2 + \frac{32\eta}{\mu \beta}e^{\frac{\beta \ell R^2}{8}}}$

Then,
\begin{align*}
a =\frac{2\xi}{\beta} \ge \frac{(R_1 - R) R_1}{\beta} = \frac{32\eta}{\mu \beta^2}e^{\frac{\beta \ell R^2}{8}}
\end{align*}
and 
\begin{align*}
(2a)^{-1/2} &\le (\frac{64\eta}{\mu \beta^2}e^{\frac{\beta \ell R^2}{8}})^{-1/2}\\
&\le \frac{1}{8}\sqrt{\frac{\mu}{\eta}} \beta e^{-\frac{\beta \ell R^2}{16}}\\
&\le \sqrt{\frac{\mu}{\eta}} \frac{2}{\ell R^2} e^{-1}
\end{align*}
Then, we have the following inequality:
\begin{align*}
\frac{1}{1-e^{-a/2}} &\le  \max\left\{ \frac{4}{a}, \frac{1}{1-e^{-1}}\right\}\\
&\le  \max\left\{ \frac{\mu \beta^2 }{8 \eta} e^{-\frac{\beta \ell R^2}{8}}, \frac{1}{1-e^{-1}}\right\}
\end{align*}
which uses the fact that for all $y>0$, $\frac{1}{1-e^{-y}} \le \max\left\{ \frac{2}{y}, \frac{1}{1-e^{-1}}\right\}$
and see the proof detail in \citep{lamperski2021projected}.

So 
\begin{align*}
1+ \frac{2 \varphi(R)^{-1}}{1-e^{-a/2}} \le 1+ 2 e^{\frac{\beta \ell R^2}{8}}\max\left\{ \frac{\mu \beta^2 }{8 \eta} e^{-\frac{\beta \ell R^2}{8}}, \frac{1}{1-e^{-1}}\right\}
\end{align*}

Without loss of generality, we assume that $\frac{a}{2} \ge 1$, which leads to $\frac{1}{1-e^{-a/2}} \le \frac{1}{1-e^{-1}} $  
% I am not sure about it. -Yuping

Then, we have 
$$c_{\ref{contraction_const1}} = 2 e^{\beta \ell R^2/8}\sqrt{\frac{2}{\mu}\left( (\ell +\mu)R^2 + R \|\nabla_x \bar{f}(0)\| + \frac{n}{\beta}\right)}$$

$$
c_{\ref{contraction_const2}} = 4 e^{\beta \ell R^2/8}
$$

\begin{align*}
c_{\ref{error_polyhedron1}} &= \left(c_{\ref{AtoC1}}+c_{\ref{BoundCtoD2}}\sqrt{c_{\ref{AlgBound}}}+ \sqrt{2} c_{\ref{BoundCtoD3}} \right) e^{\ell}\left( 1+  \frac{2\varphi(R)^{-1}}{1-e^{-\frac{16\eta}{\mu \beta^2}e^{\frac{\beta \ell R^2}{8}}}}\right) \\
& \le \left(c_{\ref{AtoC1}}+c_{\ref{BoundCtoD2}}\sqrt{c_{\ref{AlgBound}}}+ \sqrt{2} c_{\ref{BoundCtoD3}} \right) e^{\ell}\left(1+ \frac{2e^{\frac{\beta \ell R^2}{8}}}{1-e^{-1}}\right)
\end{align*}

\begin{align*}
c_{\ref{error_polyhedron2}} &= \left( 6(\frac{1}{\alpha})^{\textrm{rank}(A)/2}+1\right) \sqrt{2\ell^2}e^{\ell}\left( 1+ \frac{2 e^{\beta \ell R^2/8}}{1-e^{-\frac{16\eta}{\mu \beta^2}e^{\frac{\beta \ell R^2}{8}}}}\right)\\
& \le \left( 6(\frac{1}{\alpha})^{\textrm{rank}(A)/2}+1\right) \sqrt{2\ell^2}e^{\ell} \left(1+ \frac{2e^{\frac{\beta \ell R^2}{8}}}{1-e^{-1}}\right)
\end{align*}


This is the bound we want to simplify:
\begin{align*}
%  \label{eq:mainBound2}
  W_1(\cL(\bx_T), \pi_{\beta \bar{f}}) &\le
  \left( c_{\ref{contraction_const1}} + c_{\ref{contraction_const2}} \sqrt{\varsigma} + \frac{c_{\ref{error_polyhedron1}} + c_{\ref{error_polyhedron2}}\sqrt{\varsigma}}{(2a)^{1/2}} \right)  T^{-1/2} \log T\\
  &\le  \left( c_{\ref{contraction_const1}} + c_{\ref{contraction_const2}} \sqrt{\varsigma} + {c_{\ref{error_polyhedron1}} + c_{\ref{error_polyhedron2}}\sqrt{\varsigma}}\sqrt{\frac{\mu}{\eta}} \frac{2}{\ell R^2} e^{-1} \right)  T^{-1/2} \log T .
\end{align*}

Observing the main constants in the bound gives
\begin{align*}
%  \label{eq:mainBound2}
  W_1(\cL(\bx_T), \pi_{\beta \bar{f}}) 
  \le    p(\beta^{-1/2})e^{\beta \ell R^2/8} T^{-1/2} \log T .
\end{align*}
where $p(\beta^{1/2})$ is a polynomial function.

We assume $\beta >1$, then
\begin{align*}
%  \label{eq:mainBound2}
  W_1(\cL(\bx_T), \pi_{\beta \bar{f}}) 
  \le    p(1)e^{\beta \ell R^2/8} T^{-1/2} \log T .
\end{align*}

We want to get the sufficient condition for
$$uW_1(\cL(\bx_T), \pi_{\beta \bar{f}}) \le \frac{\epsilon}{2}.$$

For all $\delta \in (0, 1) $, 
$T^{-1/2} \log T \le \sqrt{\frac{T^{-1 +\delta}}{e \delta}}  $.
% How to pick the range of \delta? -Yuping

So it suffices to have

\begin{equation}
T^{-1+\delta} \le e\delta (\epsilon /2)^2 (u p(1) e^{\frac{\beta \ell R^2}{8}})^{-2} := \hat \epsilon
\end{equation}

so 
\begin{align*}
T &\ge \hat \epsilon^{-\frac{1}{1-\delta}}\\
 &= \left(\frac{4 e^{-1} u^2 p(1)^2}{\delta \epsilon} \right)^{\frac{1}{1-\delta}} e^{\frac{\beta \ell R^2}{16(1-\delta)}}
\end{align*}

Let $\rho = \frac{2}{1-\delta} > 2$ since $\delta <1$.

Then we have 
\begin{align*}
T &\ge \hat \epsilon^{-\frac{1}{1-\delta}}\\
 &= \left(\frac{\rho 4 e^{-1} u^2 p(1)^2}{\rho-2  }\right)^{\rho/2} \frac{1}{\epsilon^\rho}  e^{\frac{\rho\beta \ell R^2}{32}}
\end{align*}


\end{proof}

==> nearOptimality_further.tex <==
\section{Near-optimality of Gibbs distributions}

In this appendix, we prove Proposition~\ref{prop: app_optimization} which shows that $\bx_k$ can be near-optimal. The proof closely follows \cite{lamperski2021projected} and \cite{raginsky2017non}. The main difference is that in our case we have to deal with the unbounded polyhedral constraint, while in \cite{raginsky2017non} there is no constraint and in \cite{lamperski2021projected} the constraint is compact.

Firstly, we need a preliminary result shown as below.
\const{const_subopt}
\begin{lemma}
  \label{lem:gibbsSuboptimality}
Assume $\bx$ is drawn according to $\pi_{\beta \bar f}$. There exists a positive constant $c_{\ref{const_subopt}}$ such that the following bounds hold:
\begin{align*}
\bbE[\bar f(\bx)] \le \min_{x \in \cK} \bar f(x) +\frac{n}{ \beta} \left( c_{\ref{const_subopt}} + \log n \right)
\end{align*}
where $c_{\ref{const_subopt}} = 2 \log( \varsigma +\frac{1}{\mu} c_{\ref{LyapunovConst}} ) +  \frac{1}{6}\log 3 + \log 2 \sqrt{\pi} -   \log r_{\min}$.
\end{lemma}

\paragraph{Proof of Lemma~{\ref{lem:gibbsSuboptimality}}}
Recall that the probability measure $\pi_{\beta \bar f (A)}$ is defined by $\pi_{\beta \bar f (A)}(A) = \frac{\int_{A \cap \cK} e^{-\beta \bar f(x)}dx}{\int_{\cK} e^{- \beta \bar f(y)}dy}$.

Let $\Lambda = \int_{\cK} e^{-\beta \bar f(y)} dy $ and $p(x) = \frac{e^{-\beta \bar f(x)}}{\Lambda}$. So  $\log p(x) =  -\beta \bar f(x) - \log \Lambda$, which implies that $\bar f(x) = -\frac{1}{\beta} \log p(x) -\frac{1}{\beta} \log \Lambda$. Then we have
\begin{align}
\nonumber
\bbE_{\pi_{\beta \bar f}} [\bar f(\bx)] &=  \int_{\cK}  \bar f(x) p(x) dx \\
\label{eq:sub_optimal}
 &=  -\frac{1}{\beta} \int_{\cK} p(x) \log p(x) dx -\frac{1}{\beta} \log \Lambda.
\end{align}

We can bound the first term by maximizing the differential entropy. 

Let $h(x) = - \int_{\cK} p(x) \log p(x) dx$. Using the fact that the differential entropy with a finite moments is upper-bounded by that of a Gaussian density with the same second moment (see Theorem 8.6.5 in \cite{cover2012elements}), we have 
\begin{align}
\label{eq:diff_entropy_bound}
h(x) \le \frac{n}{2}\log(2 \pi e \sigma^2) \le \frac{n}{2}\log(2 \pi e ( \varsigma +\frac{1}{\mu} c_{\ref{LyapunovConst}})),
\end{align}
where $\sigma^2 = \bbE_{\pi_{\beta\bar f}}[\|\bx\|^2]$ and 
the second inequality uses Lemma \ref{lem:continuousBound}.

We aim to derive the upper bound of the second term of (\ref{eq:sub_optimal}).

First we show that there is a vector $x^\star \in \cK$ which minimizes $\bar f$ over $\cK$. In other words, an optimal solution exists. The bound (\ref{eq:quadraticLower}) from the proof of Lemma~\ref{lem:gibbs} implies that $\bar f(x)\ge  \bar f(0)+1$ for all sufficiently large $x$. This implies that there is a compact ball, $B$ such that if $x_n\in \cK$ is a sequence such that $\lim_{n\to \infty}\bar f(x_n)=\inf_{x\in\cK} \bar f(x)$, then $x_n$ must be in $B\cap \cK$ for all sufficiently large $n$. Then since $\bar f$ is continuous and $B\cap \cK$ is compact, there must be a limit point $x^\star \in B\cap \cK$ which minimizes $\bar f$. 


Let $x^* \in \cK$ be a minimizer. The normalizing constant can be expressed as:
%The existence of $x^*$ comes from the closeness of $\cK$   (??, 
%Existence of minimizer?)
\begin{align*}
\label{eq:logNormalizationConstant}
\log \Lambda &= \log \int_{\cK} e^{-\beta \bar f(x)} dx\\
	&= \log e^{-\beta \bar f(x^*)} \int_{\cK} e^{\beta \left( \bar f(x^*) - \bar f(x)\right) } \\
	&= -\beta \bar f(x^*) + \log  \int_{\cK} e^{\beta \left( \bar f(x^*) - \bar f(x)\right) } dx
\end{align*}
%The trick follows \cite{lamperski2021projected}.

So, to derive our desired upper bound on $-\log\Lambda$, 
it suffices to derive a lower bound on $\int_{\cK} e^{\beta \left( \bar f(x^*) - \bar f(x)\right) } dx$.


We have 
\begin{align*}
\bar f(x) - \bar f(x^*) =  \int_0^1 \nabla \bar f(x^* + t(x-x^*))^\top (x-x^*)dt.
\end{align*} 
Let $y = x^* + t(x-x^*)$, $t \in [0,1]$, then
\begin{align*}
\|\nabla \bar f(y)\| &= \| \nabla \bar f(y) - \nabla \bar f(x^*) +  \nabla \bar f(x^*) - \nabla \bar f(0) + \nabla \bar f(0)\| \\
 &\le \ell \| y- x^*\| + \ell \| x^*\|  + \| \nabla \bar f(0)\| \\
 & \le \ell \|x-x^*\| t + \ell \| x^*\|  + \| \nabla \bar f(0)\|.
\end{align*}

We can show $\|x^*\|$ is upper bounded by $\max \{R, \frac{\nabla \|\bar f(0)\|}{\mu}\}$. 

We have to find the bound for the case $\|x^*\| > R$.

The convexity outside a ball assumption gives
\begin{equation}
\label{eq:conv_opt}
\left( \nabla \bar f(x^*) - \nabla \bar f(0) \right)^\top x^* \ge \mu \|x^*\|^2.
\end{equation}

The optimality of $x^*$ gives $-\nabla \bar f(x^*) \in N_{\cK}(x^*)$, which is to say for all $y \in \cK$, $-\nabla \bar f(x^*)^\top (y- x^*) \le 0$. Since $0 \in \cK$, $\nabla \bar f(x^*)^\top x^* \le 0 $ holds. Applying the Cauchy-Schwartz inequality to the left hand side of \eqref{eq:conv_opt} gives 
\begin{align*}
 \| \nabla \bar f(0) \|  \|x^*\| \ge \mu \|x^*\|^2.
\end{align*}

\const{xoptBound}
This implies that $\|x^*\| \le  \frac{\|\nabla \bar f(0)\|}{\mu}  $. So we can conclude that $\|x^*\| \le \max \{R,  \frac{\|\nabla \bar f(0)\|}{\mu} \} = c_{\ref{xoptBound}}$.

Therefore,
\begin{align*}
\bar f(x) - \bar f(x^*) &\le \int_0^1 \|\nabla \bar f(y)\| \|x -x^*\| dt \\
&\le \frac{\ell}{2} \|x- x^*\|^2 + \left( \ell \| x^*\|  + \| \nabla \bar f(0)\|\right) \|x-x^*\| \\
&\le \frac{\ell}{2} \|x- x^*\|^2 + \left( \ell c_{\ref{xoptBound}} + \| \nabla \bar f(0)\|\right) \|x-x^*\|.
\end{align*}

Here we set
\begin{align*}
&e^{\beta \left( \bar f(x^*) - \bar f(x)\right)}  \ge 1/2 \\
\iff &\beta \left( \bar f(x^*) - \bar f(x)\right) \ge -\log 2 \\
\impliedby & -\frac{\ell}{2} \|x- x^*\|^2 - \left( \ell c_{\ref{xoptBound}}  + \| \nabla \bar f(0)\|\right) \|x-x^*\| \ge -\frac{1}{\beta} \log 2.
\end{align*}


So solving the corresponding quadratic equation and taking the positive root gives an upper bound of $\|x- x^*\|$:
\begin{align*}
\|x - x^*\| \le - \frac{1}{\ell}\left( \ell c_{\ref{xoptBound}}  + \| \nabla \bar f(0)\|\right) + \frac{1}{\ell}\sqrt{\left( \ell c_{\ref{xoptBound}}  + \| \nabla \bar f(0)\|\right)^2 + 2 \ell \frac{1}{\beta} \log 2}.
\end{align*}

So let $\epsilon =  -\frac{1}{\ell}\left( \ell c_{\ref{xoptBound}}  + \| \nabla \bar f(0)\|\right) + \frac{1}{\ell}\sqrt{\left( \ell c_{\ref{xoptBound}}  + \| \nabla \bar f(0)\|\right)^2 + 2 \ell \frac{1}{\beta} \log 2}$ and let $\cB_{x^*}(\epsilon)$ be the ball of radius $\epsilon$ centered at $x^*$. Then we want to find a ball $\cS$ such that 
\begin{align*}
\int_{\cK} e^{\beta \left( \bar f(x^*) - \bar f(x)\right)} dx \ge \frac{1}{2} \textrm{vol} (\cK \cap \cB_{x^*}(\epsilon)) \ge \frac{1}{2} \textrm{vol}(\cS).
\end{align*}

To find the desired ball $\cS$, we consider the problem of finding the largest ball inscribed within $\cK\cap \bB_{x^\star}(\epsilon)$. This is a Chebyshev centering problem, and can be formulated 
as the following convex optimization problem.

  \begin{subequations}
    \label{eq:chebyOptimization}
  \begin{align}
    &\max_{r,y} && r \\
    \label{eq:ballInPolyhedron}
    &\textrm{subject to} && Ay \le b - r \boldsymbol{1} \\
    \label{eq:ballInBall}
    &&&\|x^* -y\| + r  \le \epsilon
  \end{align}
\end{subequations}
where $r$ and $y$ denotes the radius and the center of the Chebyshev ball respectively. The particular form arises because the rows of $A$ are unit vectors, and so the ball of radius $r$ around $y$ is inscribed in $\cK$ if and only if (\ref{eq:ballInPolyhedron}) holds, while this ball is contained in $\bB_{x^\star}(\epsilon)$ if and only if (\ref{eq:ballInBall}) holds. 
 
% The first constraint ensures that the Chebyshev ball is contained in the polyhedral constraint set and the second constraint ensures the $\epsilon$ ball is contained in the polyhedral constraint.


We rewrite this optimization problem as:
  \begin{subequations}
    \label{eq:chebyOptimization2}
  \begin{align}
    &\min_{r,y }&& -r + I_S(x^*, [r,y]^\top) \\
    &\textrm{subject to} && Ay \le b - r \boldsymbol{1}
  \end{align}
\end{subequations}

where $S = \{(x^*, [r,y^\top]^\top) \vert \|x^* -y\| + r <\epsilon \}$.

Here, $I_S$ is defined by
\begin{equation}
I_S(x,[r,y^\top]^\top ) =  \left\{ 
  \begin{array}{ c l }
    +\infty & \quad \textrm{if } (x,[r,y^\top]^\top) \notin S \\
    0                 & \quad \textrm{otherwise}.
  \end{array}
\right.
\end{equation}

Let $g(x^\star)$ denote the optimal value of (\ref{eq:chebyOptimization2}). We will show that there is a positive constant $r_{\min}>0$ such that $-g(x) \ge r_{\min}$ for all $x \in \cK$. As a result, for any $x^\star$ the corresponding Chebyshev centering solutions has radius at least $r_{\min}$. 

% To get a lower bound on the radius of this inscribed ball, we will show that the smallest possible value of the incribed radius occurs at one of the extreme points of the lineality space of $\cK$, and show that at each extreme point a ball of positive radius can be inscribed. Since $\cK$ is polyhedral, its lineality space has only finitely many extreme points, and the minimal radius for $\cS$ ha a positive lower bound. We will denote this minimal radius as $r_{\min}$.
%(A minmax problem. We want $S \in \cK \cap \cB_{x^*}(\epsilon) $ all the time, so we choose the minimum ball among all the inscribed balls. However, we also want to have a tight lower bound, which is why we pick the inscribed ball.)


Let $F(x^*,[r,y^\top]^\top)=  -r + I_s(x^*, [r,y^\top]^\top)$.  We can see that $F$ is convex in $(x^*, [r,y^\top]^\top)$  and $\textrm{dom}\:F = S$.

Let $C = \{ [r,y^\top ]^\top \vert [\boldsymbol{1} \; A] [r,y]^\top  \le b \}$. Then the optimal value of (\ref{eq:chebyOptimization2}) can be expressed as $g(x)= \inf_{[r,y^\top ]^\top \in C} F(x, [r,y^\top]^\top)$ and $\textrm{dom}\:g = \{ x \vert \exists [r,y^\top]^\top \in C \; \textrm{s.t.} \; (x, [r,y^\top ]^\top) \in S\}$. 

The results of Section 3.2.5 of \cite{boyd2004convex} imply that if $F$ is convex, $S$ is convex, and $g(x) >-\infty$ for all $x$, then $g$ is also convex. 



%If $x \in \cK$, then setting $y= x$, $r =0$ gives $\|x-y\|  + r \le \epsilon$, which implies that $(x, [r,y]^\top)\in S$. So $\cK \subset \textrm{dom} \: g $.

If $(x, [r,y^\top ]^\top)\in \textrm{dom} \:F$, then 
\begin{align*}
\|x-y\| + r \le \epsilon & \implies r \le \epsilon - \|x-y\|\\
& \implies -r \ge - \epsilon + \|x-y\| > - \infty.
\end{align*}
In particular, if there exist $ y,r $ such that $(x, [r,y^\top ]^\top) \in \textrm{dom} \:F$, then $\inf_{[r,y^\top ]^\top \in C} F(x, [r,y^\top]^\top) \ge -\epsilon $.

There are two cases:
% one is such $[r,y]^\top \in C$, the other is that such $[r,y]^\top \notin C$.
\begin{itemize}
\item If there exist $[r,y^\top]^\top \in C$ such that $(x, [r,y^\top]^\top) \in \textrm{dom}\: F$, then $\inf_{[r,y^\top]^\top \in C} F(x, [r,y^\top]\top)  $ is finite and bounded below.
\item If there does not exist $[r,y^\top]^\top \in C$ such that $(x, [r,y^\top]^\top) \in \textrm{dom} \:F$, then for all $[r,y^\top]^\top \in C$, $F(x, [r,y^\top]^\top) = +\infty$. So $g(x) = \inf_{[r,y^\top]^\top\in C} F(x,[r,y^\top]\top) = +\infty > - \infty$.
\end{itemize}




Hereby, we can conclude that for all $x$ , $g(x) >-\infty$, so $g(x)$ is convex. 

%If $(x,[r,y]^\top) \notin S$, then $f(x^*,[r,y]^\top) = +\infty$.
%So for all $x^*$, minimum occurs when $(x,[r,y]^\top) \in S$, i.e. $\|x^* -y\| + r \le \epsilon$. 
%
%This is to say $-r \ge - \epsilon$, so $g(x^*) \ge - \epsilon$. Therefore, $g(x^*) \ge - \infty$ since $\epsilon$ is finite positive number.
%
%Hereby, we conclude that $g(x^*)$ is convex.

So, to found a lower bound on the inscribed radius, we want to maximize $g(x)$ over $\cK$.
%which uses \cite{rockafellar2015convex} Corollary 32.3.4.
Specifically, we analyze the following optimization problem
\begin{subequations}
    \label{eq:chebyOptimization3}
  \begin{align}
    &\max_{x \in \cK }&& g(x) 
    % &\textrm{subject to} && Ax\le b - r \boldsymbol{1}
  \end{align}
\end{subequations}
which corresponds to maximizing a convex function over a convex set. 

Note that $\cK \subset \dom{(g )}$. In particular, if $x\in\cK$, then $(x,[0,x^\top]^\top)\in S$, which implies that  $g(x) \le 0$. Thus, $g(x)\le 0$  for all $x\in \cK$. 
%
Therefore, using Theorem 32.2 \cite{rockafellar2015convex}, given $\cK$ is closed convex by our assumption and $g(x)$ is bounded above gives
\begin{align*}
\sup \left\{ g(x) \vert x \in \cK \right\} = \sup \left\{ g(x) \vert x \in E \right\}
\end{align*} 
where $E$ is a subset of $\cK$ consisting of the extreme points of $\cK \cap L^{\perp}$, where $L$ is the linearity space of $C$ and $L = \{x \vert Ax = 0  \} = \cN(A)$.

Now, we will show that $E$ is a finite set.

Let 
\begin{align*}
A = \begin{bmatrix}
U_1 & U_2
\end{bmatrix}
\begin{bmatrix}
\Sigma & 0 \\
0& 0 
\end{bmatrix}
\begin{bmatrix}
V_1^\top \\
 V_2^\top
\end{bmatrix},
\end{align*}

%This is based on SVD.
then $\cN(A) =  L = \cR(V_2)$
and $L^\perp = \cR(V_1)$, and 
\begin{align*}
K\cap L^\perp = \{ V_1 Z_1 \vert A V_1 Z_1 \le b \}. 
\end{align*}

This is a polyhedral with no lines so has a finite set of extreme points, i.e. $E$ is finite.
%
%By standard second cone programming, we can calculate the optimization one by one. Here, we set the smallest radius as $r_{\min}$. 
Then, based on the process shown in \cite{lamperski2021projected}, we  have $\textrm{vol}(\cS)\ge \frac{\pi^{n/2}}{\Gamma(n/2+1)}r_{\min}^n $, using the fact that a ball of radius $\rho$ has volumn given by $\frac{\pi^{n/2}}{\Gamma(n/2+1)}\rho^n$

Then, utilizing an upper bound of Gamma function recorded in \cite{ramanujan1988lost} shown as below:  

\begin{equation}
\label{eq:stirling}
\Gamma(x+1) < \sqrt{\pi} \left( \frac{x}{e}\right)^x \left( 8x^3 + 4x^2 +x + \frac{1}{30}\right)^{1/6}, \; x \ge 0.
\end{equation}


Setting $x = \frac{n}{2}$ in (\ref{eq:stirling}) gives:
\begin{equation}
\Gamma(\frac{n}{2}+1) < \sqrt{\pi} \left( \frac{n}{2e}\right)^{\frac{n}{2}} \left( n^3 + n^2 + \frac{n}{2} + \frac{1}{30}\right)^{1/6}.
\end{equation}

Therefore, we can find the lower bound of $\log \frac{1}{2} \textrm{vol}(S)$:
\begin{align}
\nonumber
\log \frac{1}{2} \textrm{vol}(S) &= \log \frac{\pi^{n/2}}{\Gamma(n/2+1)}r_{\min}^n - \log 2\\
\nonumber
&> \frac{n}{2} \log \pi + n \log r_{\min} - \log \left\{ \sqrt{\pi} \left( \frac{n}{2e}\right)^{\frac{n}{2}} \left( n^3 + n^2 + \frac{n}{2} + \frac{1}{30}\right)^{1/6} \right\} - \log 2\\\nonumber
\label{eq:logvolumn_bound}
&= -\frac{1}{2}  \log \pi + n \log r_{\min} + \frac{n}{2} \log (2 \pi e)  - \frac{n}{2} \log n- \frac{1}{6} \log \left( n^3 + n^2 + \frac{n}{2} + \frac{1}{30}\right) - \log 2\\
& > n \log r_{\min} + \frac{n}{2} \log (2 \pi e)  - \frac{n}{2} \log n -\frac{1}{6} \log \left(  3 n^3 \right) - \log (2 \sqrt{\pi})
\end{align}

The last inequality holds because  $n \ge 1 $.

Plugging (\ref{eq:logvolumn_bound}) and (\ref{eq:diff_entropy_bound}) in (\ref{eq:sub_optimal}) gives
\begin{align*}
\bbE_{\pi_{\beta \bar f}} [\bar f(x)] & <  \min f(x) + \frac{n}{2 \beta} \log(2 \pi e ( \varsigma +\frac{1}{\mu} c_{\ref{LyapunovConst}})) \\
& -\frac{1}{\beta} \left(  n \log r_{\min} + \frac{n}{2} \log (2 \pi e)  - \frac{n}{2} \log n  -\frac{1}{2} \log n - \frac{1}{6}\log 3 - \log 2 \sqrt{\pi} \right)\\
&= \min f(x) +\frac{n}{2 \beta} \log( \varsigma +\frac{1}{\mu} c_{\ref{LyapunovConst}}) - \frac{1}{\beta} \left(  n \log r_{\min} - \frac{n}{2} \log n  - \frac{1}{2} \log n \right)\\
&  +
\frac{1}{\beta} ( \frac{1}{6}\log 3 + \log 2 \sqrt{\pi})\\
&\le \min f(x) +\frac{n}{ \beta} \left( c_{\ref{const_subopt}} + \log n \right)
\end{align*}
where $c_{\ref{const_subopt}} = 2 \log( \varsigma +\frac{1}{\mu} c_{\ref{LyapunovConst}} ) +  \frac{1}{6}\log 3 + \log 2 \sqrt{\pi} -   \log r_{\min}$ and the last inequality holds because $n \ge 1$.

%$$ $$ We can have the lower bound of $$\textrm{vol}(S)$. 
\hfill $\blacksquare$

\const{optimization_const1}
\const{optimization_const2}
\const{2qmomentremainder1}
\const{2qmomentremainder2}
\begin{proposition} \label{prop: app_optimization}
Let $\bx_k$ be the iterates of the algorithms and assume $\eta \le \frac{\mu}{3\ell^2}$ and $\bbE[\|\bx_o\|^{2q}] < \infty$ for all $q>1$. There exist positive constants $c_{\ref{const_subopt}}, c_{\ref{optimization_const1}}, c_{\ref{optimization_const2}}$ such that for all $q>1$ and integers $k \ge 0$, the following bound holds:
\begin{align*}
\bbE[\bar f(\bx_k)] \le \min_{x \in \cK} \bar f(x) + c_{\ref{optimization_const1}} W_1(\cL(\bx_k), \pi_{\beta \bar f}) + c_{\ref{optimization_const2}} W_1 (\cL(\bx_k), \pi_{\beta \bar f})^{\frac{2-2q}{1-2q}} + \frac{n}{ \beta} \left( c_{\ref{const_subopt}} + \log n \right), 
\end{align*}
where
\begin{align*}
c_{\ref{const_subopt}} &= 2 \log( \varsigma +\frac{1}{\mu} c_{\ref{LyapunovConst}} ) +  \frac{1}{6}\log 3 + \log 2 \sqrt{\pi} -   \log r_{\min} \\
c_{\ref{optimization_const1}} &= \|\nabla \bar f(0)
\|
      + \ell \frac{2\left(\|\nabla \bar f(0)\|+\sqrt{\|\nabla \bar f(0)\|} + \sqrt{\mu \bar f(0)}\right)}{\mu} \\
c_{\ref{optimization_const2}} &=  \left( \frac{2 \ell }{\sqrt{\mu}} +C \right) \left( \frac{\ell }{\sqrt{\mu} (q-1)C}\right)^{\frac{2-2q}{-2q+1}} 
\end{align*}
\end{proposition}
\paragraph{Proof of Proposition~{\ref{prop: app_optimization}}}
  Let $\bx$ be drawn according to $\pi_{\beta \bar f}$. Then Lemma~\ref{lem:gibbsSuboptimality} implies:
  \begin{align}
  \label{eq:optimizationBound}
  \nonumber
    \bbE[\bar f(\bx_k)] &= \bbE[\bar f(\bx)] + \bbE[\bar f(\bx_k)-\bar f(\bx)]\\
                          &\le
    \min_{x \in \cK} \bar f(x) + \bbE[\bar f(\bx_k)-\bar f(\bx)] + \frac{n}{ \beta} \left( c_{\ref{const_subopt}} + \log n \right)   
  \end{align}
  So, it now suffices to bound $ \bbE[\bar f(\bx_k)-\bar f(\bx)]$. Ideally, we would bound this term via Kantorovich duality. The problem is that $\bar f$ may not be globally Lipschitz. So, we must approximate it with a Lipschitz function, and then bound the gap induced by this approximation. 

  Namely, fix a constant $m>\bar f(0)$ with $m\ge $, to be chosen later. Set $g(x)=\min\{\bar f(x),m\}$. The inequality from (\ref{eq:quadraticLower}) implies that if $\|x\|\ge \hat R:=\frac{2\left(\|\nabla \bar f(0)\|+\sqrt{\|\nabla \bar f(0)\|+\mu (m-\bar f(0))}\right)}{\mu}$,  then $\bar f(x)\ge m$. We claim that $g$ is globally Lipschitz.

  For $\|x\|\le \hat R$, we have that
  $$
  \|\nabla \bar f(x)\|\le \|\nabla \bar f(0)\| + \ell \hat R=:u.
  $$
  We will show that $g$ is $u$-Lipschitz.

  In the case that $f(y)\ge m$ and $f(x)\ge m$, we have $|g(x)-g(y)|=0$, so the property holds.
  
  Now say that $\bar f(x) < m$ and $\bar f(y) < m$. Then we must have $\|x\|\le \hat R$ and $\|y\|\le \hat R$. Then for all $t\in [0,1]$, we have $\|(1-t)x+ty \|\le \hat R$. It follows that 
  \begin{align*}
    g(x)-g(y)&= 
    \bar f(x)-\bar f(y) \\
             &= \int_0^1 \nabla \bar f(x+t(y-x))^\top (y-x) dt \\
    &\le u \|x-y\|.
  \end{align*}
  Finally, consider the case that $\bar f(x) \ge m$ and $\bar f(y) < m$. Then there is some $\theta \in [0,1]$ such that $\bar f(y + \theta (x-y))=m$. Furthermore
  \begin{align*}
    |g(x)-g(y)| &= m-\bar f(y) \\
                &= \bar f(y+\theta (x-y))-\bar f(y) \\
                &=\int_0^\theta \nabla \bar f( y + t(x-y))^\top (x-y) dt\\
                &\le u \|x-y\|.
  \end{align*}
  It follows that $g$ is $u$-Lipschitz.

  Now noting that $g(x)\le \bar f(x)$ for all $x$ gives
  \begin{align}
    \nonumber
    \bbE[\bar f(\bx_k)-\bar f(\bx)]&\le \bbE[\bar f(\bx_k)-g(\bx)] \\
    \nonumber
                                   &=\bbE[g(\bx_k)-g(\bx)] + \bbE[\indic(\bar f(\bx_k) > m) (\bar f(\bx_k)-m)] \\
    \label{eq:kantorovichSplit}
                                   &\le u W_1(\cL(\bx_k),\pi_{\beta \bar f}) + \bbE[\indic(\bar f(\bx_k) > m) (\bar f(\bx_k)-m)].
  \end{align}
  The final inequality uses Kantorovich duality. Now, it remains to bound
  $
  \bbE[\indic(\bar f(\bx_k) > m) (\bar f(\bx_k)-m)].
  $


  
  Note that if $\by$ is a non-negative random variable, a standard identity gives that $\bbE[\by]=\int_0^\infty \bbP(\by > \epsilon)d\epsilon$. Thus, we  have
  $$
  \bbE[\indic(\bar f(\bx_k) > m) (\bar f(\bx_k)-m)] = \int_0^\infty \bbP(\bar f(\bx_k) -m > \epsilon)d\epsilon.
  $$

  For all $x\in \cK$, we have
  \begin{align*}
    \bar f(x) &= \bar f(0) - \nabla \bar f(0)^\top x + \int_0^1 (\nabla \bar f(tx)-\nabla \bar f(0))^\top x dt \\
    &\le \bar f(0) +  \|\nabla \bar f(0)\| \|x \| + \frac{1}{2} \ell \|x\|^2 \\
    &\le \bar f(0) + \frac{\|\nabla \bar f(0)\|^2}{2\ell} + \ell \|x\|^2.
  \end{align*}

  So, 
  \begin{align*}
    \bar f(x)-m > \epsilon &\implies  \bar f(0) + \frac{\|\nabla \bar f(0)\|^2}{2\ell} + \ell \|x\|^2 > m+\epsilon \\
    &\iff \|x\|^2 > \frac{m+\epsilon-  \left(\bar f(0) + \frac{\|\nabla \bar f(0)\|^2}{2\ell}\right)}{\ell}.
  \end{align*}

  Now assume that $m/2 > \bar f(0) + \frac{\|\nabla \bar f(0)\|^2}{2\ell}$. Then the right side implies $\|x\|^2 \ge \frac{\frac{m}{2}-\epsilon}{\ell}$.  
%
  It follows that for any $q>1$, we have, via Markov's inequality and direct computation:
  \begin{align*}
    \bbE[\indic(\bar f(\bx_k) > m) (\bar f(\bx_k)-m)] & \le \int_0^{\infty} \bbP\left(\|\bx_k\|^2 >  \frac{\frac{m}{2}+\epsilon}{\ell} \right) d\epsilon \\
                                                      &= \int_0^{\infty} \bbP\left(\|\bx_k\|^{2q} >  \left(\frac{\frac{m}{2}+\epsilon}{\ell}\right)^q \right) d\epsilon  \\
                                                      &\le \bbE[\|\bx_k\|^{2q}] \int_0^{\infty} \left(\frac{\frac{m}{2}+\epsilon}{\ell}\right)^{-q} d\epsilon \\
    &= \bbE[\|\bx_k\|^{2q}] \frac{\ell^q 2^{q-1}}{(q-1)m^{q-1}}. 
  \end{align*}

  Plugging this expression into (\ref{eq:kantorovichSplit}) and using the definition of $u$ gives
  \begin{align}
  \label{eq:kantorovichSplit2}
    \MoveEqLeft
    \nonumber
    \bbE[\bar f(\bx_k)-\bar f(\bx)] \\
    & \nonumber
      \le \left(\|\nabla \bar f(0)
\|
      + \ell \frac{2\left(\|\nabla \bar f(0)\|+\sqrt{\|\nabla \bar f(0)\|+\mu (m-\bar f(0))}\right)}{\mu} \right) W_1(\cL(\bx_k),\pi_{\beta \bar f}) \\
    &\qquad +  \bbE[\|\bx_k\|^{2q}] \frac{\ell^q 2^{q-1}}{(q-1)m^{q-1}}.
  \end{align}


We want to derive the bound of $\bbE[\|\bx_k\|^{2q}]$.

We have
\begin{align*}
\|\bx_{k+1}\|^{2q} \le \|\bx_k - \eta \nabla f(\bx_k, \bz_k) + \sqrt{\frac{2\eta}{\beta}} \hat{\bw}_k\|^2.
\end{align*}

For notation simplicity, let $y = \frac{\bx_k - \eta \nabla f(\bx_k, \bz_k)}{\sqrt{2\eta /\beta}}$ and $w = \hat{\bw}_k$, so the above inequality can be expressed as 
\begin{align*}
\|\bx_{k+1}\|^{2q} &\le \left( \frac{2 \eta}{\beta}\right)^q\|y + w\|^{2q}\\
&= \left( \frac{2 \eta}{\beta}\right)^q \left( \|y\|^2 + \|w\|^2 +2 y^\top w \right)^q\\
&= \left( \frac{2 \eta}{\beta}\right)^q \sum_{k=0}^q  \binom qk \left( 2 y^\top w \right)^{q-k}\left( \|y\|^2 + \|w\|^2 \right)^k   \\
& = \left( \frac{2 \eta}{\beta}\right)^q \sum_{k=0}^q   \binom qk \left( 2 y^\top  w \right)^{q-k} \sum_{i=0}^k \binom ki\left( \|y\|^{2i} \|w\|^{2(k-i)}    \right).
\end{align*}

The last two equalities use binomial theorem. Taking expectation, we can observe that the right hand side bound can be expressed as $\left( \frac{2 \eta}{\beta}\right)^q \bbE\left[ \|y\|^{2q} \right] + \bbE\left[ p(\|y\|)\right]$, where $p(\|y\|)$ is a polynomial in $y$ with order strictly lower than $2q$. Note that $p(\|y\|)$ will be dominated by the higher order term if $y$ is big.
More specifically, the lower order terms will be dominated when $\bx_k$ is big. When $\bx_k$ is small, these terms can be bounded above by a constant.

So now we want to examine $\bbE[\|y\|^{2q}]$, which is to bound $\bbE[\|\bx_k - \eta \nabla \bar{f}(\bx_k)\|^{2q}]$.
We have 
\begin{align*}
\|\bx_k - \eta \nabla f(\bx_k, \bz_k)\|^{2q} &= \left( \|\bx_k\|^2 - 2 \eta \bx_k^\top \nabla f(\bx_k, \bz_k) + \eta^2 \|\nabla f(\bx_k, \bz_k)\|^2\right)^q 
%&=\|\bx_k\|^{2q} + (- 2 \eta \bx_k^\top \nabla f(\bx_k, \bz_k))^q + \eta^{2q} \| \nabla f(\bx_k, \bz_k) \|^{2q} + p_2(\|\bx_k\|).
\end{align*}
We examine the second term:
\begin{align*}
\bx_k^\top \nabla f(\bx_k, \bz_k) &= \bx_k^\top (\nabla \bar{f}(\bx_k) - \nabla \bar{f}(0)) + \bx_k^\top( \nabla \bar{f}(0) - \nabla \bar{f}(\bx_k) + \nabla f(\bx_k, \bz_k) ) \\
&\ge \mu \|\bx_k\|^2 - (\ell+ \mu) R^2 + \bx_k^\top(\nabla \bar{f}(0) + \bbE_{\hat \bz}[\nabla f(\bx_k, \bz_k) - \nabla f(\bx_k, \hat \bz_k) ])
\end{align*} 
where the first term is bounded by the assumption of the strong convexity outside a ball and the detailed statement is shown below:

If $\|x\| \ge R$, then $x^\top (\nabla \bar f(x) - \nabla \bar  f(0)) \ge \mu \|x\|^2$.

If $\|x\| \le R$, then $x^\top (\nabla \bar f(x) - \nabla \bar  f(0)) \ge - \ell \|x\|^2 \ge - \ell R^2$.

Therefore, we have for all $x \in \cK$, $x^\top (\nabla \bar f(x) - \nabla \bar f(0)) \ge \mu \|x\|^2 - (\ell+\mu) R^2$.

Note here and below $\hat \bz$ is independent of $\bz$ and identically distributed.

Then, we have
\begin{align}
\nonumber
& \bbE\left[ \|\bx_k - \eta \nabla f(\bx_k, \bz_k)\|^{2q} \right] \nonumber \\
\nonumber
&= \bbE\left[\left( \|\bx_k\|^2 - 2 \eta \bx_k^\top \nabla f(\bx_k, \bz_k) + \eta^2 \|\nabla f(\bx_k, \bz_k)\|^2\right)^q\right] \\
\nonumber
&\le \bbE\left[\left((1- 2 \mu \eta) \|\bx_k\|^2 + 2 \eta (\ell+ \mu) R^2  \right.\right. \\ \nonumber & \left. \left. \qquad - 2 \eta\bx_k^\top(\nabla \bar{f}(0) + \bbE_{\hat \bz}[\nabla f(\bx_k, \bz_k) - \nabla f(\bx_k, \hat \bz_k) ]) + \eta^2 \|\nabla f(\bx_k, \bz_k)\|^2\right)^q\right] \\
\nonumber
&\le \bbE\left[\left((1- 2 \mu \eta) \|\bx_k\|^2 + 2 \eta (\ell+ \mu) R^2  \right.\right. \\ \nonumber & \left. \left. \qquad - 2 \eta\bx_k^\top(\nabla \bar{f}(0) + \nabla f(\bx_k, \bz_k) - \nabla f(\bx_k, \hat \bz_k) ) + \eta^2 \|\nabla f(\bx_k, \bz_k)\|^2\right)^q\right] \\
 \nonumber
&\le \bbE\left[\left((1- 2 \mu \eta) \|\bx_k\|^2 + 2 \eta (\ell+ \mu) R^2  \right.\right. \\  & \left. \left. \qquad + 2 \eta \|\bx_k\|(\|\nabla \bar{f}(0)\| +  \ell(\bz_k -  \hat \bz_k) ) + \eta^2 \|\nabla f(\bx_k, \bz_k)\|^2\right)^q\right]. 
\label{eq:Bound2qmoment}
\end{align}

The second inequality uses Jensen's inequality, and the last inequality uses Cauchy-Schwartz inequality together with $\ell$-Lipschitzness of $\nabla f(x,z)$ in $z$.

Now we examine the last term above.
\begin{align*}
\|\nabla f(x,z)\| &= \|\nabla f(x,z) - \bbE_{\hat{z}}[\nabla f(x, \hat z)] + \bbE_{\hat z}[\nabla f(x, \hat z)]\| \\
&\le \|\bbE_{\hat{z}}[ \nabla f(x,z) - \nabla f(x, \hat z)]\| + \| \bar{f}(x)\| \\
&\le \ell \bbE_{\hat{z}}[ \|z - \hat z\|] + \|\nabla \bar{f}(0)\| + \ell \|x\|.
\end{align*}
So
\begin{align}
\label{eq:fsquareBound}
\|\nabla f(x,z)\|^2 \le 3 \left( \ell^2 \left(\bbE_{\hat{z}}[ \|z - \hat z\|] \right)^2 + \|\nabla \bar{f}(0)\|^2 + \ell^2 \|x\|^2\right).
\end{align}

Then, we can group the square terms in (\ref{eq:Bound2qmoment}) together and simplify it:
\begin{align*}
&(1-2\mu \eta) \|x\|^2 + \eta^2 3 \ell^2 \|x\|^2 \le (1-\eta \mu) \|x\|^2\\
\iff & 1-2\mu \eta + \eta^2 3 \ell^2 \le 1- \eta \mu \\
 \iff& \eta \le \frac{\mu}{3\ell^2}.
\end{align*}

So, if $\eta \le \frac{\mu}{3\ell^2}$,  plugging (\ref{eq:fsquareBound}) into (\ref{eq:Bound2qmoment}) gives 
\begin{align*}
\bbE\left[ \|\bx_k - \eta \nabla f(\bx_k, \bz_k)\|^{2q} \right] &\le \bbE\left[\left((1- \mu \eta) \|\bx_k\|^2 + 2 \eta (\ell+ \mu) R^2  \right.\right. \\  & \left. \left. - 2 \eta \|\bx_k\|(\|\nabla \bar{f}(0)\| +  \ell(\bz_k -  \hat \bz_k) ) + \eta^2 3 \left( \ell^2 \left(\bbE_{\hat{\bz}}[ \|\bz_k - \hat \bz_k\|] \right)^2 \|\nabla \bar{f}(0)\|^2 \right) \right)^q\right].
\end{align*}

We want to further group the first and third terms above together.

Let $a= \|\bx_k\|$, $b = \|\nabla \bar{f}(0)\| +  \ell(\bz_k -  \hat \bz_k) $. For all $\epsilon \ge 0$, $2ab = 2 (\epsilon a) (\frac{1}{\epsilon} b) \le (\epsilon)^2 + (\frac{1}{\epsilon}b)^2$ .

Then, we have
\begin{align*}
&(1- \mu \eta) \|\bx_k\|^2 + \eta \epsilon^2 \|\bx_k\|^2
\le (1- \frac{\mu \eta}{2}) \|\bx_k\|^2 \\
\iff & 1- \mu \eta +\eta \epsilon^2 \le 1- \frac{\mu \eta}{2} \\
\iff & \epsilon \le \sqrt{\frac{\mu}{2}}.
\end{align*}

So let $\epsilon = \sqrt{\frac{\mu}{2}}$, we have
\begin{align*}
\bbE\left[ \|\bx_k - \eta \nabla f(\bx_k, \bz_k)\|^{2q} \right] &\le \bbE\left[\left((1- \frac{\mu \eta}{2}) \|\bx_k\|^2 + 2 \eta (\ell+ \mu) R^2  \right.\right. \\  & \left. \left. + \frac{2\eta}{\mu}(\|\nabla \bar{f}(0)\| +  \ell(\bz_k -  \hat \bz_k) )^2 + \eta^2 3 \left( \ell^2 \left(\bbE_{\hat{\bz}}[ \|\bz_k - \hat \bz_k\|] \right)^2 \|\nabla \bar{f}(0)\|^2 \right) \right)^q\right] \\
&\le \bbE\left[\left((1- \frac{\mu \eta}{2}) \|\bx_k\|^2 + 2 \eta (\ell+ \mu) R^2  \right.\right. \\  & \left. \left. + \frac{2\eta}{\mu}(\|\nabla \bar{f}(0)\| +  \ell(\bz_k -  \hat \bz_k) )^2 + \eta^2 3 \left( \ell^2 \left( \|\bz_k - \hat \bz_k\| \right)^2 \|\nabla \bar{f}(0)\|^2 \right) \right)^q\right] \\
& = (1-\frac{\mu \eta}{2})^q \bbE[\|\bx_k\|^{2q}] + \eta \bbE[p(\|\bx_k\|^2, \|\bz_k -\hat{\bz}_k\|^2)]\\
&\le (1-\frac{\mu \eta}{2}) \bbE[\|\bx_k\|^{2q}] + \eta \bbE[p(\|\bx_k\|^2, \|\bz_k -\hat{\bz}_k\|^2)]\\
& \le (1- \frac{\mu \eta}{4}) \bbE[\|\bx_k\|^{2q}] + \eta \bbE[-\frac{\mu}{4} \|\bx\|^{2q} + p(\|\bx_k\|^2, \|\bz_k -\hat{\bz}_k\|^2)]\\
&\le (1- \frac{\mu \eta}{4}) \bbE[\|\bx_k\|^{2q}] + \eta c_{\ref{2qmomentremainder1}}.
 \end{align*}

The second inequality uses Jensen's inequality twice.
The polynomial $p(\|\bx_k\|^2, \|\bz_k -\hat{\bz}_k\|^2)$ is with order strictly lower than $2q$ in $\|\bx_k\|$ and with highest order of $2q$ in $\|\bz - \hat{\bz}_k\|$. The last inequality is based on the claim that $\bbE[-\frac{\mu}{4} \|\bx\|^{2q} + p(\|\bx_k\|^2, \|\bz_k -\hat{\bz}_k\|^2)]$ is bounded by a constant $c_{\ref{2qmomentremainder1}}$, which depends on the value of $q$, the statistics of external random variables $\bz$.
%We can calculate this constant value out.

Therefore, we have 
\begin{align*}
\bbE[\|\bx_{k+1}\|^{2q}] \le (1-\frac{\eta \mu}{4}) \bbE[\|\bx_k\|^{2q}] + \eta c_{\ref{2qmomentremainder2}}.
\end{align*}

Intuitively, the constant $c_{\ref{2qmomentremainder2}}$ represents the influence of the lower order remainders in the processes of using binomial theorem.

Now as long as $\bbE[\|\bx_0\|^{2q}] < \infty$, we have
\begin{align*}
\bbE[\|\bx_k\|^{2q}] \le \bbE[\|\bx_0\|^{2q}] + c_{\ref{2qmomentremainder2}}.
\end{align*}

Plugging the above result into (\ref{eq:kantorovichSplit2}) gives 
  \begin{align*}
  \label{eq:kantorovichSplit3}
    \MoveEqLeft
    \bbE[\bar f(\bx_k)-\bar f(\bx)] \\
    &
      \le \left(\|\nabla \bar f(0)
\|
      + \ell \frac{2\left(\|\nabla \bar f(0)\|+\sqrt{\|\nabla \bar f(0)\|+\mu (m-\bar f(0))}\right)}{\mu} \right) W_1(\cL(\bx_k),\pi_{\beta \bar f}) \\
    &\qquad +  \left( \bbE[\|\bx_0\|^{2q}] + c_{\ref{2qmomentremainder2}} \right) \frac{\ell^q 2^{q-1}}{(q-1)m^{q-1}}.
  \end{align*}

The remaining work is to optimize the left hand side with respect to $m$ so that we can make a choice of the value of $m$ which is mentioned earlier in the proof.

Let 
\begin{align*}
g(m)&=\left(\|\nabla \bar f(0)
\|
      + \ell \frac{2\left(\|\nabla \bar f(0)\|+\sqrt{\|\nabla \bar f(0)\|} + \sqrt{\mu m} + \sqrt{\mu \bar f(0)}\right)}{\mu} \right) W_1(\cL(\bx_k),\pi_{\beta \bar f}) \\
    &\qquad +  \left( \bbE[\|\bx_0\|^{2q}] + c_{\ref{2qmomentremainder2}} \right) \frac{\ell^q 2^{q-1}}{(q-1)m^{q-1}}.
  \end{align*}
We can see that $g(m)$ is an upper bound of the right hand side of (\ref{eq:kantorovichSplit2}). 
  
Setting $g^\prime(m) = 0$ leads to $m^* = \left( \frac{\ell W_1}{\sqrt{\mu} (q-1)C}\right)^{\frac{2}{-2q+1}}$, where $C = \left( \bbE[\|\bx_0\|^{2q}] + c_{\ref{2qmomentremainder2}} \right) \frac{\ell^q 2^{q-1}}{(q-1)}$ for notation simplicity. 
So 
\begin{align*}
\max_{m \ge 0}g(m) &= g(m^*)\\
&\le \left(\|\nabla \bar f(0)
\|
      + \ell \frac{2\left(\|\nabla \bar f(0)\|+\sqrt{\|\nabla \bar f(0)\|} + \sqrt{\mu \bar f(0)}\right)}{\mu} \right) W_1(\cL(\bx_k),\pi_{\beta \bar f}) \\
      & + \frac{2 \ell }{\sqrt{\mu}} \left( \frac{\ell W_1(\cL(\bx_k),\pi_{\beta \bar f})}{\sqrt{\mu} (q-1)C}\right)^{\frac{2-2q}{-2q+1}}
       +  C \left( \frac{\ell W_1(\cL(\bx_k),\pi_{\beta \bar f})}{\sqrt{\mu} (q-1)C}\right)^{\frac{2-2q}{-2q+1}}\\
       & =  \left(\|\nabla \bar f(0)
\|
      + \ell \frac{2\left(\|\nabla \bar f(0)\|+\sqrt{\|\nabla \bar f(0)\|} + \sqrt{\mu \bar f(0)}\right)}{\mu} \right) W_1(\cL(\bx_k),\pi_{\beta \bar f}) \\
      & + \left( \frac{2 \ell }{\sqrt{\mu}} +C \right) \left( \frac{\ell }{\sqrt{\mu} (q-1)C}\right)^{\frac{2-2q}{-2q+1}}
       W_1(\cL(\bx_k),\pi_{\beta \bar f})^{\frac{2-2q}{-2q+1}}
\end{align*}


%
Setting 
\begin{align*}
c_{\ref{optimization_const1}} &= \|\nabla \bar f(0)
\|
      + \ell \frac{2\left(\|\nabla \bar f(0)\|+\sqrt{\|\nabla \bar f(0)\|} + \sqrt{\mu \bar f(0)}\right)}{\mu} \\
c_{\ref{optimization_const2}} &=  \left( \frac{2 \ell }{\sqrt{\mu}} +\left( \bbE[\|\bx_0\|^{2q}] + c_{\ref{2qmomentremainder2}} \right) \frac{\ell^q 2^{q-1}}{(q-1)} \right) \left( \frac{\ell }{\sqrt{\mu} (q-1)\left( \bbE[\|\bx_0\|^{2q}] + c_{\ref{2qmomentremainder2}} \right) \frac{\ell^q 2^{q-1}}{(q-1)}}\right)^{\frac{2-2q}{-2q+1}}.
\end{align*}
and plugging this bound into (\ref{eq:optimizationBound}) give the desired result.


 Below are some further proofs that need to work on later.
\begin{align*}
(2a)^{-1/2} &\le (\frac{64\eta}{\mu \beta^2}e^{\frac{\beta \ell R^2}{8}})^{-1/2}\\
&\le \frac{1}{8}\sqrt{\frac{\mu}{\eta}} \beta e^{-\frac{\beta \ell R^2}{16}}
%&\le \sqrt{\frac{\mu}{\eta}} \frac{2}{\ell R^2} e^{-1}
\end{align*}
%The last inequality is based on the assumption that $\ell R^2 \beta \le 16$.

Therefore, we can simplify the bound in Theorem \ref{thm:nonconvexLangevin} as below
\begin{align*}
%  \label{eq:mainBound2}
  W_1(\cL(\bx_T), \pi_{\beta \bar{f}}) &\le
  \left( c_{\ref{contraction_const1}} + c_{\ref{contraction_const2}} \sqrt{\varsigma} + \frac{c_{\ref{error_polyhedron1}} + c_{\ref{error_polyhedron2}}\sqrt{\varsigma}}{(2a)^{1/2}} \right)  T^{-1/2} \log T\\
  &\le  \left( c_{\ref{contraction_const1}} + c_{\ref{contraction_const2}} \sqrt{\varsigma} + \left( c_{\ref{error_polyhedron1}} + c_{\ref{error_polyhedron2}} \sqrt{\varsigma} \right)\frac{1}{8}\sqrt{\frac{\mu}{\eta}} \beta e^{-\frac{\beta \ell R^2}{16}}\right)  T^{-1/2} \log T .
\end{align*}



Observing the main constants in the bound gives
\begin{align*}
%  \label{eq:mainBound2}
  W_1(\cL(\bx_T), \pi_{\beta \bar{f}}) 
  \le    p(\beta^{-1/2})\beta T^{-1/2} \log T .
\end{align*}
where $p(\beta^{-1/2})$ is a polynomial function.

We assume $\beta >1$, then
\begin{align*}
%  \label{eq:mainBound2}
  W_1(\cL(\bx_T), \pi_{\beta \bar{f}}) 
  \le    p(1)\beta T^{-1/2} \log T .
\end{align*}

We want to get the sufficient condition for
$$c_{\ref{optimization_const1}}W_1(\cL(\bx_T), \pi_{\beta \bar{f}}) \le \frac{\epsilon}{4}.$$

For all $\delta \in (0, 1) $, 
$T^{-1/2} \log T \le \sqrt{\frac{T^{-1 +\delta}}{(\frac{e \delta}{2})^2}}  $.
 How to pick the range of $\delta$? -Yuping

So it suffices to have

\begin{equation}
T^{-1+\delta} \le \left( \frac{e\delta}{2} \right)^2 (\frac{\epsilon}{4})^2 (c_{\ref{optimization_const1}} p(1) \beta)^{-2} := \hat \epsilon
\end{equation}

so 
\begin{align*}
T &\ge \hat \epsilon^{-\frac{1}{1-\delta}}\\
 &= \left(\frac{64}{\delta^2 \epsilon^2 e^2} \right)^{\frac{1}{1-\delta}}  (c_{\ref{optimization_const1}} p(1) \beta)^{\frac{2}{1-\delta}}
\end{align*}

Let $\rho = \frac{2}{1-\delta} > 2$ since $\delta <1$.

Then we have 
\begin{align*}
T &\ge \hat \epsilon^{-\frac{1}{1-\delta}}\\
 &= \left(\frac{\rho 8  c_{\ref{optimization_const1}} p(1)}{e(\rho-2 ) }\right)^{\rho} \frac{1}{\epsilon^\rho}  \beta^{\rho}
\end{align*}



\begin{align*}
c_{\ref{optimization_const2}} W_1 (\cL(\bx_k), \pi_{\beta \bar f})^{\frac{2-2q}{1-2q}} \le \frac{\epsilon}{4}
\end{align*}
\begin{align*}
T^{-1+\delta} \le  \left( \frac{e\delta}{2} \right)^2 (\frac{\epsilon}{4})^{\frac{1-2q}{1-q}} c_{\ref{optimization_const2}}^{-\frac{1-2q}{1-q}} (p(1) \beta)^{-2}:= \hat \epsilon
\end{align*}
\begin{align*}
T \ge \left( \left( \frac{e\delta}{2} \right)^2 (\frac{\epsilon}{4})^{\frac{1-2q}{1-q}} c_{\ref{optimization_const2}}^{-\frac{1-2q}{1-q}} (p(1) \beta)^{-2} \right)^{-\frac{1}{1-\delta}}:= \hat \epsilon
\end{align*}
Let $\rho = \frac{2}{1-\delta} > 2$ since $\delta <1$.

\begin{align*}
T\ge \left( \frac{2 \rho p(1) \beta}{e (\rho -2)} \right)^{-\rho} \epsilon^{\frac{1-2q}{1-q} \frac{\rho}{ 2}} \left( 4 c_{\ref{optimization_const2}}\right)^{-\frac{1-2q}{1-q} \frac{\rho}{2}}
\end{align*}
where $c_{\ref{optimization_const2}}$ depends on $q$ and the initial $2q$ moment of $\bx$.


And let $\frac{n}{ \beta} \left( c_{\ref{const_subopt}} + \log n \right) \le \frac{\epsilon}{2}$, we have 
\begin{align*}
\beta \ge \frac{2 n ( c_{\ref{const_subopt}} + \log n)}{\epsilon}
\end{align*}
\hfill $\blacksquare$

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> revisionClarification.tex <==
\section*{Corrections for the Main Paper}

During edits of the supplementary material after the submission of the main paper, a few minor errors were flagged. The result is that some of the constant terms in the results changed. In each case, the originally stated results actually remain true, but the work in the supplementary material derives slightly different constant factors. The differences are highlighted below. 



\paragraph*{Correction of Theorem~\ref{thm:nonconvexLangevin} and Lemma~\ref{lem:AtoC}} Theorem~\ref{thm:nonconvexLangevin} remains true. In the original paper, we required that $\eta\le \min\left\{\frac{1}{4},\frac{\mu}{8\ell^2} \right\}$. In the supplemental material, we show that the theorem holds as long as  $\eta$ satisfies the slightly weaker bound of $\eta\le \min\left\{\frac{1}{4},\frac{\mu}{4\ell^2} \right\}$.

Similarly, Lemma~\ref{lem:AtoC}, which is used to prove Theorem~\ref{thm:nonconvexLangevin}, required $\eta\le \min\left\{\frac{1}{4},\frac{\mu}{8\ell^2} \right\}$ in the original submission. In the supplemental material, we show that the lemma holds as long as $\eta\le \min\left\{\frac{1}{4},\frac{\mu}{4\ell^2} \right\}$. 

\paragraph*{Correction of Lemma~\ref{lem:MeanBetween1}}
% \label{lem:MeanBetween1}
{\it 
  For all $s\ge 0$ and all $k\ge 0$, the following bound holds:
  \begin{equation*}
          \nonumber
%          \MoveEqLeft[0]
          W_1\left(\cL(\bx_k^{M,s}),\cL(\bx_k^{B,s}) \right)
          \le \bbE[\|\bx_k^{M,s}-\bx_k^{B,s}\|] 
    \le   2\ell \psi_2(s,\bz)\eta \sqrt{k} .
  \end{equation*}
}

In the submission, Lemma~\ref{lem:MeanBetween1} has the looser upper bound
$$
          W_1\left(\cL(\bx_k^{M,s}),\cL(\bx_k^{B,s}) \right)
          \le \bbE[\|\bx_k^{M,s}-\bx_k^{B,s}\|] 
    \le   2\ell \left(\psi_2(s,\bz)+\psi_2(s+1,\bs)\right)\eta \sqrt{k} .
$$

The bound from Lemma~\ref{lem:MeanBetween1} was used to derive Lemma~\ref{lem:MeanBetween2}, and as a result this must be corrected to:

\paragraph*{Correction of Lemma~\ref{lem:MeanBetween2}}
{\it
%\label{lem:MeanBetween2}
For all $s\ge 0$ and all $k\ge 0$, the following bound holds
%\begin{equation*}
\begin{multline}
 \nonumber
  W_1\left(\cL(\bx_k^{B,s}),\cL(\bx_k^{M,s+1})\right) \le \bbE[\|\bx_k^{B,s}-\bx_k^{M,s+1}\|]  
  \le
  2\ell \psi_2(s,\bz)\eta \sqrt{k} \left( e^{\eta k \ell}-1\right).
\end{multline}
}

The bounds from Lemma~\ref{lem:MeanBetween1} and \ref{lem:MeanBetween2} were used to prove Lemma~\ref{lem:AtoCdependent}. The proof with the corrected bounds is given below. 

\paragraph*{Corrected proof of Lemma~\ref{lem:AtoCdependent}}
  Recalling that $\bx_k^{M,0}=\bx_k^A$ and $\bx_k^{M,k+1}=\bx_k^M$ and using the triangle  inequality gives:
  \begin{align}
    \nonumber
    \MoveEqLeft[0]
    W_1(\cL(\bx_k^A),\cL(\bx_k^M))
    \\
    \nonumber
    &\le
      \sum_{s=0}^{k} W_1(\cL(\bx_k^{M,s}),\cL(\bx_k^{M,s+1}))\\
    \nonumber
    &\le \
      \sum_{s=0}^{k} \left(W_1(\cL(\bx_k^{M,s}),\cL(\bx_k^{B,s})) +
      W_1(\cL(\bx_k^{B,s}),\cL(\bx_k^{M,s+1}))\right)\\
    \nonumber
    &\overset{\textrm{Lemmas~\ref{lem:MeanBetween1}~\& ~\ref{lem:MeanBetween2}}}{\le}
      \sum_{s=0}^{k}2\ell\psi_2(s,\bz)\eta \sqrt{k}e^{\eta\ell k}
    \\
    \label{eq:AtoMdependent}
    &\le 2\ell \Psi_2(\bz) \eta \sqrt{k}e^{\eta \ell k}.
  \end{align}
  Here $\psi_2(s,\bz)$ and $\Psi_2(\bz)$ are the terms that bound the decay of probabilistic dependence between the $\bz_k$ variables, as defined in \eqref{eq:LMixing}.

  Similarly, we bound
  \begin{align}
    \nonumber
    \MoveEqLeft[0]
    W_1(\cL(\bx_k^M),\cL(\bx_k^C))\\
    \nonumber
    &\le W_1(\cL(\bx_k^M),\cL(\bx_k^D))+W_1(\cL(\bx_k^D),\cL(\bx_k^C))
    \\
    \label{eq:MtoCdependent}
    &\overset{\textrm{Lemmas}~\ref{lem:C2D}~\&~\ref{lem:M2D}}{\le}
       \left( (c_{\ref{BoundCtoD1}} + c_{\ref{BoundCtoD2}} \sqrt{\varsigma}) \eta \sqrt{k} + c_{\ref{BoundCtoD3}} \sqrt{\eta \log(4k)} \right) e^{\eta\ell k}.
  \end{align}
  Plugging the bounds from (\ref{eq:AtoMdependent}) and (\ref{eq:MtoCdependent}) into (\ref{eq:AtoCTriangle}) proves the lemma, with $c_{\ref{AtoC1}} = \AtoCOneVal $.
  \hfill$\blacksquare$

%\end{equation*}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

